Synthesizing Stellar Populations in South Pole Telescope Galaxy Clusters: I. Ages of Quiescent Member Galaxies at 0.3 < z < 1.4

Using stellar population synthesis models to infer star formation histories (SFHs), we analyse photometry and spectroscopy of a large sample of quiescent galaxies which are members of Sunyaev-Zel'dovich (SZ)-selected galaxy clusters across a wide range of redshifts. We calculate stellar masses and mass-weighted ages for 837 quiescent cluster members at 0.3 < z < 1.4 using rest-frame optical spectra and the Python-based Prospector framework, from 61 clusters in the SPT-GMOS Spectroscopic Survey (0.3 < z < 0.9) and 3 clusters in the SPT Hi-z cluster sample (1.25 < z < 1.4). We analyse spectra of subpopulations divided into bins of redshift, stellar mass, cluster mass, and velocity-radius phase-space location, as well as by creating composite spectra of quiescent member galaxies. We find that quiescent galaxies in our dataset sample a diversity of SFHs, with a median formation redshift (corresponding to the lookback time from the redshift of observation to when a galaxy forms 50% of its mass, t$_{50}$) of $z=2.8\pm0.5$, which is similar to or marginally higher than that of massive quiescent field and cluster galaxy studies. We also report median age-stellar mass relations for the full sample (age of the Universe at $t_{50}$ (Gyr) = $2.52 (\pm0.04) - 1.66 (\pm0.11)$ log$_{10}(M/10^{11} M\odot))$ and recover downsizing trends across stellar mass; we find that massive galaxies in our cluster sample form on aggregate $\sim0.75$ Gyr earlier than lower mass galaxies. We also find marginally steeper age-mass relations at high redshifts, and report a bigger difference in formation redshifts across stellar mass for fixed environment, relative to formation redshifts across environment for fixed stellar mass.

==> graveyard.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Flow of Argument:
% 1. Stellar Population in Massive Passive Galaxies is the key to understanding mass assembly and quenching processes.
% 2. Field Galaxy Work recently -- CLEAR, MOSDEF, VANDELS -- has pushed the envelope of studying these objects to z ~ 1-3. Quiescent galaxies at this epoch are truly well-assembled galaxies, and potential progenitors of low-z objects.
%3. Environmental dependence is a topic of study - one of the environments where passive galaxies are readily available are galaxy clusters. Limited number of galaxy cluster studies to link stellar populations across a wide range of masses and redshifts (CNOC, LoCUSS, WINGS, ICBS, GOGREEN).
%4. My sample is special - because galaxy clusters are selected on the basis of non-optical properties, and high-z clusters can be linked to low-z clusters in a descendant-antecedent manner in an SZ-selected (and hence mass-limited) sample. 
%5.  Preamble to this work, and the science questions it answers.
%

%
%August 26th: \NOTE{Agenda here:\\
%1. Stellar Population in Galaxies tell us about formation and evolution pathways of galaxies.\\
%2. Field Galaxy work exists, traditionally photometry.\\
%3. Recent work has shown that spectroscopy is much better at calculating ages, especially with rest frame optical indicators.\\
%4. Moreover limited spectrophotometry work that studies environments. Those who do (e.g. cluster environment) do not have unbiased samples - cannot do descendant-antecedent studies.\\ 
%5. My work has photometry, spectroscopy, and an unbiased and representative cluster sample.}

%How and whether a given galaxy undertakes the path from initial star formation, quenching, to passive evolution thereafter, is a fundamental question in the field of galaxy evolution. Studies that characterize galaxy mass assembly as a function of stellar content, halo mass, and environment are a path forward in both defining and solving the problem. In the last two decades, synthesizing stellar populations in galaxies via photometry-based spectral energy distributions (SEDs) has been recognized as a path forward to measure stellar masses, ages, and metallicities of a diverse population of galaxies.

%In spite of tremendous progress, studies relying on photometry alone are subject to many challenges, such as the age-metallicity-dust degeneracy (see Worthey 1994, and Charlot \& Silk 1999). With the advent of spectroscopic surveys and measurements of spectral features that are robust age indicators (e.g. H$\delta$ in absorption, and the d4000 spectral index), our ability to infer physical properties of galaxies from SED fitting has significantly improved. Moreover, recent complex numerical simulations have been able to reproduce many physical conditions of galaxies and demonstrate hierarchical structure formation (e.g. Springel et al. 2005, TNG/SIMBA Simulation; \NOTE{REF}), as well as approximately infer the parameters of evolution required to connect high-redshift galaxies to low-redshift objects. But refining this process, including adding physically motivated quenching mechanisms to simulations, and testing these simulations against representative galaxy samples as a function of redshift, stellar mass and environment, are tasks that still remain. 

%Studying massive galaxies across cosmic time is a robust path towards understanding the processes that govern the formation and evolution of all galaxies. Recent multi-wavelength photometric surveys have been successful in studying complete samples upto z>3 (e.g. CLEAR, VANDELS, MOSFIRE -- \GK{Cite everything laid out in Page 2, VANDELS Carnall et al. 2019}  Panter, Heavens \& Jimenez 2003; Cimatti et al. 2004, 2008; Heavens et al. 2004; Daddi et al. 2005; Gallazzi et al. 2005, 2014; Panter et al. 2007; Onodera et al. 2012, 2015; Jørgensen \& Chiboucas 2013; Whitaker et al. 2013; Choi et al. 2014; Citro et al. 2016; Fumagalli et al. 2016; Pacifici et al. 2016; Siudek et al. 2017; Carnall et al. 2018; Belli, Newman \& Ellis 2019; Estrada-Carpenter et al. 2019; Carnall et al. 2019, 2020)). These observations have confirmed that the number density of massive passive galaxies in the field has increased by $\sim$1 dex since z$\sim$2 (Ilbert et al. 2013, Muzzin et al. 2013, Fumagalli et al. 2016), and that quenching processes (environmental,...) are responsible for decreasing the star formation rates (SFRs) in these galaxies. Numerous studies discuss both the timescales of cessation of star formation, and the likely process/processes responsible for quenching, noting that the efficacy of these processes is a strong function of environmental phenomena (e.g. ram pressure stripping, etc.) 

%While large samples of galaxy photometry exist ranging from the present epoch to z $\sim$ 2-3 for L*-type (and fainter) galaxies (CANDELS REF), only recently do we have access to detailed spectroscopic datasets across billions of years, allowing us to ask questions of how typical galaxies at low redshift become descendents of galaxies (see Dressler 2016 -- diversity of SFHs, and references therein). Moreover, this framework of a 'longitudinal' analysis has been applied even fewer times for member galaxies of clusters, for which you need a robust non-optically-selected galaxy cluster sample (see CNOC, WINGS, LoCuSS, ICBS surveys).

%Recent studies of modest heterogeneous samples of galaxy clusters at $1 < z < 2$ have shown high star formation and active galactic nuclei (AGN) activity compared with lower redshifts, and a luminosity function that is evolving \citep{2009ApJ...697..436H,2010ApJ...720..284M,2012ApJ...761..141M,2010ApJ...719L.126T,2011NJPh...13l5014F,2012ApJ...756..114S,2012ApJ...756..115Z,2013ApJ...779..138B,2014MNRAS.437..437A,2016ApJ...825...72A}. This is evidence that galaxy clusters are undergoing significant mass assembly in this epoch, inviting further investigation into properties of member galaxies and the intra-cluster medium (ICM) at $z > 1$.

%Studies that analyze cluster galaxies (both as individual objects and in aggregate) at $z < 1$ suggest that galaxies in clusters form stars in an epoch of early and rapid star formation (at $z > 3$), before quickly settling into a mode of passive and stable evolution (Dressler and Gunn 1982, Balogh et al. 1999, Dressler et al. 2004), 1998ApJ...492..461S,2005ApJ...634L.129S,2005ApJ...620L..83H,2006ApJ...644..759M). Thus, observations of clusters at higher redshifts should sample an epoch where this star formation --- or at least its end stages --- is observed \textit{in situ}.  \NOTE{Star formation in galaxies, and dependence on environment, e.g. galaxy clusters. This paragraph needs to be REWRITTEN and elaborated upon further.}

%Recently we have seen studies conducted with galaxy cluster environments compared with field galaxies, to chart the role that these dense environments and deep gravitational potential wells play in the transition of galaxies from star-forming to passive (ICBS, CNOC, GOGREEN Webb et al. 2019). These studies characterize ages and star formation histories of massive passive and star forming galaxies, and infer quenched fractions of galaxies in these environments, but the cluster samples are either optical or infrared selected objects, with significant bias in cluster section while studying the very optical properties we are determined to characterize in member galaxies e.g. studying galaxies in `rich' clusters as was the case with the ICBS cluster sample. 

%Discovery of clusters in the high-redshift Universe is still technically challenging. This is due to two main reasons. First, optical, IR and X-ray fluxes -- which are observational tracers of galaxy clusters -- become progressively more difficult to measure at high redshift due to cosmological dimming. Second, to conduct evolutionary studies and characterize the precursors of lower-redshift clusters, we need to study the appropriate higher-redshift antecedents of lower-redshift massive clusters which are lower-mass systems, which is a non-trivial sample to build. Third, a challenge with optical and IR cluster surveys is whether the selection of galaxy clusters based on member galaxy properties — i.e. flux — systematically affects the studies of those member galaxy properties. These challenges are mitigated by clusters discovered via the Sunyaev-Zel'dovich (SZ) effect. Clusters discovered with the South Pole Telescope (SPT) and the Atacama Cosmology Telescope (ACT) provide a nearly redshift-independent, mass-limited sample of clusters with a mass threshold set by instrument sensitivity (Carlstrom et al. 2002).

%Matt: maybe add a sentence at the start of this paragraph saying that recent 
% SZ-based galaxy cluster searches have revealed new samples of galaxy clusters at z$\sim$1-2? 
% maybe cite this: https://ui.adsabs.harvard.edu/abs/2002ARA\%26A..40..643C/abstract ?

%It is well-established from studies of modest heterogenous samples of galaxy clusters at $1 < z < 2$ (that have shown high star formation and active galactic nucleus (AGN) activity) that galaxy clusters are undergoing significant mass assembly in this epoch (Hilton et al. 2009; Tran et al. 2010; Fassbender et al. 2011; Snyder et al. 2012; Brodwin et al. 2013; Alberts et al. 2014, 2016). Moreover, recent SZ-based galaxy cluster searches have revealed new samples of galaxy clusters at z$\sim$1-2 (Huang et al. 2020, Bleem et al. 2020, ACT REF). 

%The 2500 deg$^{2}$ South Pole Telescope Sunyaev-Zel'dovich (SPT-SZ) survey catalog contains 677 galaxy cluster candidates with a statistical significance $>$ 4.5, with 37 at $z > 1$ (Bleem et al. 2015, hereafter B15) based primarily on photometric red-sequence redshifts. Spectroscopic confirmations along with astrophysical and cosmological analyses of multiple high redshift and massive galaxy clusters from the SPT-SZ survey, many unique to the SPT-SZ sample, have been previously published \citep{2010ApJ...721...90B, 2013ApJ...763...93S, 2014ApJ...792...45R, 2014ApJ...794...12B, 2016ApJS..227....3B, 2013ApJ...774...23M, 2017arXiv170205094M}. Optical and infrared spectrophotometric data in these surveys sample galaxy over-densities and are successful in probing low cluster halo mass thresholds for systems with a breadth of star formation histories.



%Much work has focused on understanding quenching mechanisms better, and to chart the pathways that a galaxy takes to reach the passive evolution stage. Environmental quenching takes place either due to ram pressure stripping, or by preventing the formation of new star in a galaxy by stopping cold gas accretion (Gun \& Gott 1972, Balogh, Navarro and Morris 2000). AGN-feedback processes are thought to play a major role in quenching (Dave, Thompson and Hopkins 2016, Dace et al. 2019, Nelson et al. 2019). An environment where observations to test these scenarios are readily available are galaxy clusters, with an abundance of passively evolving galaxies.




%Galaxy formation and evolution in rich environments like groups and clusters..... With the advent of high-resolution spectroscopic and precise photometric data and robust spectral energy distribution (SED) models, several questions in the field of galaxy evolution can be answered. 

%Abramson et al. 2018 (and references therein) situate challenges in the endeavour of studying galaxy evolution precisely -- data captures systems at different times (i.e. no real-time evolution is seen in galaxies, of course) while the physical phenomena affecting the systems operate on a given system over different epochs. This may not be true at the level of characterizing aggregate physical phenomena at the level of galaxy population, especially at the margins of datasets e.g. the faintest red galaxies, member galaxies in cluster environments, etc. \NOTE{WHY IS THIS NOT TRUE??}



